Visual Anomaly Detection in Event Sequence Data

Anomaly detection is a common analytical task that aims to identify rare cases that differ from the typical cases that make up the majority of a dataset. When applied to the analysis of event sequence data, the task of anomaly detection can be complex because the sequential and temporal nature of such data results in diverse definitions and flexible forms of anomalies. This, in turn, increases the difficulty in interpreting detected anomalies. In this paper, we propose an unsupervised anomaly detection algorithm based on Variational AutoEncoders (VAE) to estimate underlying normal progressions for each given sequence represented as occurrence probabilities of events along the sequence progression. Events in violation of their occurrence probability are identified as abnormal. We also introduce a visualization system, EventThread3, to support interactive exploration and interpretations of anomalies within the context of normal sequence progressions in the dataset through comprehensive one-to-many sequence comparison. Finally, we quantitatively evaluate the performance of our anomaly detection algorithm and demonstrate the effectiveness of our system through a case study.

==> sections/03-overview.tex <==
\section{System Overview}
\label{sec:overview}
Our system is designed to support interactive exploration and interpretation of anomalies in event sequence data. The designs were iteratively improved over four months of regular discussions with an expert who investigates anomaly detection problems and works closely with professionals in various fields, such as health informatics, social media, and urban computing. We identified the following design requirements for detecting anomalies in event sequences from the expert's feedback and our experience with event sequence analysis.

\begin{itemize}
    \item[\textbf{R1}]\textbf{Noise removal and feature extraction.} 
    The system should be able to filter out unimportant variation of event types to allow for higher quality subsequent analysis.

    \item[\textbf{R2}]\textbf{Anomalous sequence detection.} 
    Real-world event sequence datasets are often large and rarely contain labels. The system should incorporate an unsupervised anomaly detection mechanism for the anomalous sequences to narrow users' inspection on the detected outliers rather than the entire dataset.
    
    \item[\textbf{R3}]\textbf{Anomalous event localization.} 
    The interpretation of the detected anomalous sequences relies on the analysis of low-level events. However, real-world event sequences can be long in length and heterogeneous in types, which makes it difficult to identify abnormality on event level. Therefore, the system should be able to highlight anomalous events within the abnormal sequences to facilitate reasoning and interpretation.
    
    \item[\textbf{R4}]\textbf{Sequence exploration and interpretation in contexts.}
    Analyzing anomalies within the context of normal progressions can help reveal higher-level anomalous patterns (e.g., anomalous sub-sequences, anomalous event ordering) beyond anomalous events and provide insights for interpretation. The system should provide users with an interactive environment to explore sequence dataset and analyze anomalous sequences within the context of normal progressions to help interpret the anomalies.

\end{itemize}

Motivated by these requirements, we developed \name, an interactive visualization system for detecting and visualizing anomalies in temporal event sequences. As illustrated in Fig.~\ref{fig:system_overview}, the system includes (1) a data preprocessing module, (2) an anomaly detection module, and (3) a visualization module. The data preprocessing module removes noisy events with small TF-IDF scores~\cite{guo2018eventthread} and exclude extremely short sequences (i.e., sequence length $<$ 2), so as to prepare high-quality event sequence data for training the anomaly detection model (\textbf{R1}). In the analysis module, we identify anomalous sequences (\textbf{R2}) and uncover event occurrence probabilities of normal progressions from a trained LSTM-VAE. We further localize anomalous events within the detected outliers by referring to the occurrence probabilities of each event in normal progressions (\textbf{R3}). The analysis results are then sent to the visualization module for interactive visual analysis of the anomalous sequences via multi-granular sequence exploration and data comparison (\textbf{R4}).

\begin{figure}[t!]
\centering
\includegraphics[width=\columnwidth]{figures/system_overview.png}
\vspace{-1.5em}
\caption{The \name system pipeline.}
\label{fig:system_overview}
\vspace{-1.5em}
\end{figure}
